Simulating Liquidity: Agent-Based Modeling of Illiquid Markets for Fractional Ownership

This research investigates liquidity dynamics in fractional ownership markets, focusing on illiquid alternative investments traded on a FinTech platform. By leveraging empirical data and employing agent-based modeling (ABM), the study simulates trading behaviors in sell offer-driven systems, providing a foundation for generating insights into how different market structures influence liquidity. The ABM-based simulation model provides a data augmentation environment which allows for the exploration of diverse trading architectures and rules, offering an alternative to direct experimentation. This approach bridges academic theory and practical application, supported by collaboration with industry and Swiss federal funding. The paper lays the foundation for planned extensions, including the identification of a liquidity-maximizing trading environment and the design of a market maker, by simulating the current functioning of the investment platform using an ABM specified with empirical data.

==> Empirical_Results/Tables/Cluster_Description.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{l: l: l: l}

         & Cluster 0 & Cluster 1 & Cluster 2 \\ \hline
        \textit{Number of assets} & 10 & 4 & 5 \\ \hdashline
        \textit{Number of trades} & 777 & 759 & 522 \\ \hdashline
       \textit{Median relative price} & -0.04\% & 3.17\% & -4.07\% \\ \hdashline
        \textit{Mean relative price} & -0.27\% & 3.48\% & -4.28\% \\ \hline
        ~ & ~ & ~ & ~ \\ \
       \textbf{Buy side, relative} & ~ & ~ & ~ \\ \hdashline
        \textit{  Buyer trades} & 70\% & 73\% & 48\% \\ \hdashline
        \textit{  Buyer \& Seller trades} & 30\% & 27\% & 52\% \\ \hline
        ~ & ~ & ~ & ~ \\ 
       \textbf{Sell side, relative} & ~ & ~ & ~ \\ \hdashline
        \textit{  Seller trades} & 72\% & 58\% & 91\% \\ \hdashline
        \textit{  Buyer \& Seller trades} & 28\% & 42\% & 9\% \\ \hline
    \end{tabular}
    \caption{Descriptive analysis of clusters}
    \label{tab:Descriptive_Analysis_of_Clusters}
\end{table}

==> Notes.tex <==
This chapter presents details on data processing (\autoref{subsec:Sample_Reduction_&_Market_Aggregation}) and the specification of the ABM underlying the simulation of the operational platform of the FinTech company (\autoref{subsec:ABM}).

\subsection{Sample reduction \& market aggregation}\label{subsec:Sample_Reduction_&_Market_Aggregation}


Given the presence of 154 different assets, with some having only a few observations, an aggregation based on their similarity in relative price changes, i.e. specifically, the percentage deviation of the price paid for a Splint relative to its last available valuation, is conducted. This approach attempts to result in homogeneous markets of similarly traded assets, helping to address small sample size problems for individual assets and reduce complexity for the simulations to be run.

The aggregation of the individual asset markets is performed using a $k$-means clustering approach, utilizing the mean and median relative price paid for all trades on the secondary market for each asset. To determine the optimal number of clusters, the silhouette score, a measure for evaluating the cohesion and separation of clusters, is calculated for different numbers of possible clusters. The number of clusters that results in the maximum silhouette score is considered optimal. The corresponding results are discussed in \autoref{subsec:clustering_results}.

To ensure the reliability of mean and median values on which the clustering is based, only assets with at least 30 Splints traded during the observation period are considered.\footnote{Note that most trades have a trade size of one Splint. Those trades that comprise more than one Splint were broken down into several trades with a trade size of one in an intermediate step. This step simplifies modelling and simulation, as the trade size is identical for all transactions.} This step reduces the number of in-scope assets from 154 to 19. Overall, these 19 assets account for 2,058 Splints traded, or 48 percent of all Splints trades conducted on the Splint platform over the total sample period.

The remaining trades reveal that there are 201 users that only sell, 302 that only buy, and 62 users that buy and sell on the secondary market. The ABM to be implemented is grounded in these three agent types and the economic behavior drivers that influence them.

\subsection{ABM}\label{subsec:ABM}

The simulation of the underlying market structure models three agent types based on empirical findings: pure sellers, pure buyers, and agents who can both buy and sell assets. The specification of the agents is described in the following.

\subsubsection{Pure seller}

The pure seller initiates selling if it experiences an exogenous liquidity-shock in iteration $i$ that happens with probability $p$. In case of a shock, the seller decides to sell all its assets. The seller is also endowed with a discount factor $d$, which is a shape parameter of the agent's pricing function. A higher discount factor implies that the agent is willing to sell its assets at lower prices.

The pricing decision of the assets are based on a triangular distribution with a probability density function (PDF) of the form

%\textcolor{red}{discuss notation here}

\begin{equation*}
    p(x)= 
    \begin{cases}
        \frac{2(x-\underline{v})}{(mode-\underline{v})(\overline{v}-\underline{v})} & \underline{v}<x \leq mode \\
        \vspace{3pt} \\
        \frac{2(\overline{v}-x)}{(\overline{v}-\underline{v})(\overline{v}-mode)} & mode<x<\overline{v},
    \end{cases}
\end{equation*}
where:
    \begin{itemize}
        \item $mode$ is the reference valuation times $1-d$ where $d$ is a discount factor,
        \item $\underline{v}$ is the minimum possible valuation (75\% of the reference valuation),
        \item and $\overline{v}$ is the maximum possible valuation (110\% of the reference valuation).
    \end{itemize}

The minimum possible and maximum possible offer price as well as the asset valuation are exogenous and based on the setup of the platform of the FinTech company.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Pure buyer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The pure buyer can only buy assets in the market. This agent is motivated by partly emotional motivation to become the owner of a rare asset. The agent is not strictly optimising his potential profit, and is therefore endowed with a generalised logistic decision function of the form
    \begin{equation*}
        p(x) = \frac{1}{1+e^{+k \cdot(x+A)}}.
    \end{equation*}
The parameters influence the behavior of the agent in the following way:

\begin{itemize}
    \item High $k$ (steep slope): The agent reacts sensitive to relative price. Small changes in price will significantly change the agent's probability of accepting or rejecting the offer.
    \item Low $k$ (gradual slope): The agent is less sensitive. Changes in relative price do not influence the agent's behavior heavily. 
    \item High $A$ (shifted right): The agent requires a higher relative price to reach the same probability of offer acceptance.
    \item Lower $A$ (shifted left): The agent requires a lower relative price to reach the same probability of offer acceptance.
\end{itemize}

%\textcolor{red}{Verify results: For buyerseller type, lower k fits better to data. For logistic buyer, higher k is more likely. Both have same level of A (zero). Use more granular optimizer}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Buyer-seller}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The third class, a mixed agent type that can buy and sell assets sequentially, is also used. The buyer-seller - in contrast to the pure buyer and pure seller - is maximizing its realized return.  


The third type of agent has a mixed strategy, where it can buy and sell assets. The agent follows an opportunistic, valuation-based strategy. For the selling of assets, the agent tries to realize profits. Therefore, the pricing decision is based on a  Weibull Maximum Extreme Value distribution.

The PDF of the Weibull Maximum Extreme Value distribution with the scale parameter \(\gamma\) and the location parameter \(\alpha\) is given by:

\[
f(x; c, \alpha, \gamma) = \frac{c}{\gamma} \left( \frac{\alpha - x}{\gamma} \right)^{c-1} \exp \left( - \left( \frac{\alpha - x}{\gamma} \right)^c \right),
\]

where:
\begin{itemize}
    \item \( x \leq \alpha \)
    \item \( c \) is the shape parameter,
    \item \( \gamma \) is the scale parameter,
    \item \( \alpha \) is the location parameter.
\end{itemize}


The interpretation of the parameters is the following:

\begin{itemize}
    \item \textbf{Shape Parameter \(c\)}: Controls the tail behavior of the distribution, where higher values lead to heavier tails (increasing the likelihood of extreme values) and lower values result in lighter tails. A higher \(c\) results in a steeper distribution concentrated around \(\alpha\), while a lower \(c\) flattens the distribution and spreads out the values, decreasing the likelihood of extremes near \(\alpha\).
    \item \textbf{Scale Parameter \(\gamma\)}: Stretches or compresses the distribution horizontally around the location parameter \(\alpha\), affecting the spread of data points. A higher \(\gamma\) makes the distribution wider, increasing variability, while a lower \(\gamma\) makes it narrower, reducing variability.
    \item \textbf{Location Parameter \(\alpha\)}: Sets the maximum possible value for the distribution, effectively shifting the entire distribution left or right. Changing \(\alpha\) shifts the maximum possible value higher or lower but does not affect the shape or the spread of the distribution.
\end{itemize}


The purchase decision of the buyer-seller is based on the same generalized logistic function used for the pure buyer, but the parameter values for these two agent types can differ.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Parameter optimization}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\textcolor{red}{write down optimization of parameters}

For the distributional parameters described in the previous section, we perform a grid randomized, iteratively narrowing grid search over the parameter space.

We optimize the Wasserstein distance between the three empirical clusters and the simulated markets in our ABM. Specifically, this approach attempts to bring the distribution of the number of trades per relative price in the simulated markets as close as possible to the corresponding empirical results. The Wasserstein distance, as a measure for comparing the similarity of probability distributions, is defined as 

\begin{equation}
\mathbb{W}_p(P, Q):=\left(\inf _{\pi_{X, Y \in \Pi(P, Q)}} \mathbb{E}_\pi\left[\|X-Y\|^p\right]\right)^{1 / p}, 
\label{eq:wasserstein_distance}
\end{equation}
where:

\begin{itemize}
    \item $P$ and $Q$ are probability distributions over a metric space.
    \item $\Pi(P, Q)$ represents the set of all joint distributions $\pi_{X, Y}$ whose marginals are respectively $P$ and $Q$.
    \item $\pi_{X, Y}$ is a particular joint distribution in $\Pi(P, Q)$ that couples $P$ and $Q$.
    \item $\mathbb{E}_\pi[\|X-Y\|^p]$ denotes the expectation of the $p$-th power of the Euclidean distance between $X$ and $Y$ under the joint distribution $\pi_{X, Y}$.
    \item $\inf_{\pi_{X, Y \in \Pi(P, Q)}}$ indicates taking the infimum over all joint distributions $\pi_{X, Y}$ in the set $\Pi(P, Q)$.
    \item $X$ and $Y$ are random variables governed by the joint distribution $\pi_{X, Y}$, where $X$ has distribution $P$ and $Y$ has distribution $Q$.
\end{itemize}

Through this distance measure, we optimize the following parameters:

\begin{itemize}
    \item \texttt{shock\_probability}: The probability that in a given iteration, a seller agent experiences an exogenous liquidity shock that leads to it trying to sell its assets.
    \item \texttt{discount\_factor}: The discount factor $d$. The higher the discount factor, the lower the mode of the distribution's mean. This implies that the agent is - on average - willing to offer its shares at a lower price.
    \item \texttt{A}: The $A$ parameter of the buyer agent.
    \item \texttt{K}: $k$ the k parameter of the buyer agent.
    \item \texttt{c\_shape}: The shape parameter of the Weibull Maximum Extreme Value distribution, i.e. the pricing function of the buyer-seller agent. %\textcolor{red}{describe influences}
    \item \texttt{scale}: The $\gamma$ scale parameter of the Weibull Maximum Extreme Value distribution. %\textcolor{red}{describe how it influences}
    \item \texttt{A\_bs}: The $A$ parameter of the buyer-seller agent.
    \item \texttt{k\_bs}: The $k$ parameter of the buyer-seller agent.
\end{itemize}

When optimizing the parameters within the parameter space w.r.t. to the Wasserstein distance in  \autoref{eq:wasserstein_distance}, we arrive at the parameters described in Table \ref{tab:optimised_params}.

\begin{table}[h]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Parameter}         & \textbf{Value}           \\ \hline
\texttt{shock\_probability} & 0.156                  \\ 
\texttt{discount\_factor}   & 0.0                      \\ 
\texttt{A}                  & -0.125                   \\ 
\texttt{K}                  & 1.532       \\
\texttt{c\_shape}           & 1.993              \\ 
\texttt{scale}              & 1.525                    \\ 
\texttt{A\_bs}              & -1.883               \\ 
\texttt{k\_bs}              & 1.525                    \\ \hline
\end{tabular}
\caption{Optimized parameters for the model}
\label{tab:optimised_params}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Markets}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The number of markets to be modelled is determined depending on the number of homogeneous asset clusters identified in the 19 remaining assets after data reduction due to the small sample size for some of the original assets (see \autoref{subsec:Sample_Reduction_&_Market_Aggregation}). The settlement of offers in the markets happens iteratively, with trades being settled for iteration $i$ for all the markets constructed. 

%We model three distinct markets to replicate the clusters of different asset types. The settlement of offers in the markets happens iteratively, with trades being settled for iteration $i$ for all the three markets. 

%\textcolor{red}{describe number of iterations, etc.}

In this chapter, the empirical results from the clustering empirical trades to generate homogenous markets (\autoref{subsec:clustering_results}) and the simulated markets (\autoref{subsec:Simulation_results}) are discussed.

\subsection{Clustering results}\label{subsec:clustering_results}
Due to the sample size issue caused by the low number of transactions relative to the number of assets, we cluster the assets to increase the available data for market simulation. Specifically, we apply $k$-means clustering to the mean and median relative prices of the 19 most frequently traded assets in the secondary market. To determine the optimal number of clusters, we calculate the Silhouette score for cluster counts ranging from 2 to 18. The corresponding results are shown in \autoref{fig:Silhouette_Scores}.


\begin{figure}[!h]
    \centering
    \includegraphics[width=\columnwidth]{6) Empirical Results/Figures/Silhouette_Scores.png}
    \caption{Silhouette scores per number of clusters}
    \label{fig:Silhouette_Scores}
\end{figure}

The figure indicates that the highest Silhouette score is achieved with three clusters, with a value of 0.56. This score suggests that the clusters are reasonably well-defined. Our market structure to be modelled below is therefore based on the assumption of three classes of similar assets.

\autoref{fig:Empirical_Clusters} illustrates the total number of Splints traded in the empirical data, categorized by relative price for the three clusters. The following conclusions can be drawn:


\begin{figure}[!h]
    \centering
    \includegraphics[width=\columnwidth]{6) Empirical Results/Figures/Empirical_Clusters.png}
    \caption{Empirical clusters of trades by relative price}
    \label{fig:Empirical_Clusters}
\end{figure}



\begin{itemize}
    \item Cluster 0: The assets in this cluster tend to be traded close to their valuation. 
    \item Cluster 1: The assets in this cluster tend to be traded above their valuation. Buyers are therefore willing to pay a markup on these assets.
    \item Cluster 2: The assets in this cluster tend to be traded below their valuation. Sellers are therefore willing to accept a discount for these assets.
\end{itemize}

More descriptive statistics on the clusters are presented in \autoref{tab:Descriptive_Analysis_of_Clusters}, detailing the number of assets, number of trades, median and mean relative prices, and the breakdown of buy and sell-side trades for each cluster.

Cluster 0 contains the most assets, totaling 10. This is followed by Cluster 2, which has 5 assets, and Cluster 1, which has 4 assets. Cluster 0 also leads in trading activity, with 777 transactions, indicating a high level of activity within this cluster. Cluster 1 follows closely with 759 trades, while Cluster 2 has the lowest trading activity, with 522 trades. 
The average and median values of the relative prices traded reinforce the findings from \autoref{fig:Empirical_Clusters}. In Cluster 0, the traded Splints are priced close to their valuation (median of $-0.04\%$; mean of $-0.27\%$). In Cluster 1, Splints are typically traded above their valuation (median of $3.17\%$; mean of $3.48\%$), whereas in Cluster 2, they are often traded below their valuation (median of $-4.07\%$; mean of $-4.28\%$).


\input{6) Empirical Results/Tables/Cluster_Description}

\autoref{tab:Descriptive_Analysis_of_Clusters} further shows the proportion of trades by user type for both the buy and sell sides within each cluster. Overall, the findings align with our assumptions about user behavior. From a buying perspective, pure Buyers are more active in Clusters 0 and 1, where prices are generally at or above valuation. This supports our assumption that pure Buyers are less price-sensitive, as they are not solely driven by profit motives. Buyers \& Sellers are most active as the buying party in Cluster 2, which aligns with our assumption of their profit-driven behavior.

From the selling perspective, pure Sellers are most active in Clusters 0 and 2, while Buyer \& Sellers have the highest proportion of sales in Cluster 1. This suggests that pure Buyers are more likely to accept discounts on assets sold, supporting our assumption that their behavior is driven by (short-term) liquidity needs. In contrast, Buyer \& Sellers tend to sell at prices above the asset's valuation, reinforcing their profit-driven behavior.

\subsection{Simulation}\label{subsec:Simulation_results}


% Since - in the empirical data - the users tend to offer smaller amounts of shares (between 1 and 5), the number of shares $n$ being put on the follows this distribution:
% \begin{equation}
%     P(n) = log_{10}(n+1) - log_{10}(n).
% \end{equation}
% When comparing the simulated distribution of the amount of shares offered in Figure \ref{fig:simulated_sharenumber_dist} to the empirical offer distribution in Figure \ref{fig:empirical_sharenumber_dist}, it becomes apparent that the simulated distribution closely matches the empirical distribution in the data. On average, the Pure Seller agent offers their assets for a lower price because he is interested in partially liquidating his portfolio.
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{3) Data/Figures/shares_offered_dist.png}
%     \caption{Sellers choose lower number of splints for their offers with higher probability}
%     \label{fig:simulated_sharenumber_dist}
% \end{figure}


\begin{algorithm}
\caption{Pure Seller's (PS) Decision to Act and Offer Assets}
\begin{algorithmic}[1]
\State \textbf{Input:} None
\State \textbf{Variables:} \textit{Splints}, \textit{Cash}
\State \textbf{Parameters:} \textit{PS\_offer\_probability}, \textit{PS\_offer\_ratio}, $a_{PS,l}$, $a_{PS,h}$, $p_{ref}$

\If{$Random(0, 1) < PS\_offer\_probability$ \textbf{and} $Splints > 0$} 
    \State $n_i \gets PS\_offer\_ratio \times Splints$ 
    \State $p_i \gets Uniform(a_{PS,l} \times p_{ref}, a_{PS,h} \times p_{ref})$
    \State Add offer $o_i = (p_i, n_i)$ to offer book $O$
\Else
    \State No action taken
\EndIf
\State \textbf{Output:} Enter an offer in the offer book or do nothing.
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Pure Buyer's (PB) Decision to Act and Buy Assets}
\begin{algorithmic}[1]
\State \textbf{Input:} Offer book $O$
\State \textbf{Pure Buyer Variables:} \textit{Splints}, \textit{Cash}
\State \textbf{Seller Agent Variables:} \textit{Splints\_seller}, \textit{Cash\_seller}
\State \textbf{Parameters:} \textit{PB\_trading\_probability}, \textit{PB\_purchase\_ratio}, $p_{ref}$, $k$

\If{$Random(0, 1) < PB\_trading\_probability$} 
    \State \parbox[t]{\linewidth}{Pick a random offer $o_i = (p_i, n_i, Seller\_Agent)$ from \\ $O$}
    
    \State \parbox[t]{\linewidth}{Calculate purchase probability $P(p_i) \gets \\ \frac{1}{1 + e^{-k(p_i - p_{ref})}}$}

    \If{$Random(0, 1) < P(p_i)$}
    
        \State \parbox[t]{\linewidth}{Calculate purchase amount $purchase\_amount \gets$ \\ $PB\_purchase\_ratio \times Cash$}
    
        \If{$purchase\_amount \geq p_i \times n_i$}
            \State \textbf{Pure Buyer:}
                \State Update \textit{Splints} to $(Splints + n_i)$
                \State Update \textit{Cash} to $(Cash - (p_i \times n_i))$
            
            \State \textbf{Seller Agent:}
                \State Update \textit{Splints\_seller} to $(Splints\_seller - n_i)$
                \State \parbox[t]{\linewidth}{Update \textit{Cash\_seller} to $(Cash\_seller + (p_i \times \\ n_i))$}

            \State Remove $o_i$ from $O$
        \Else
            \State \textbf{Pure Buyer:}
                \State \parbox[t]{.6\linewidth}{Update \textit{Splints} to $(Splints + purchase\_amount / p_i)$}
                \State Update \textit{Cash} to $(Cash - purchase\_amount)$
            
            \State \textbf{Seller Agent:}
                \State \parbox[t]{\linewidth}{Update \textit{Splints\_seller} to $(Splints\_seller - \\ (purchase\_amount / p_i))$}
                \State \parbox[t]{\linewidth}{Update \textit{Cash\_seller} to $(Cash\_seller + \\ purchase\_amount)$}

            \State Update $n_i$ to $(n_i - (purchase\_amount / p_i))$  
        \EndIf

    \Else
        \State No action taken
    \EndIf
\Else
    \State No action taken
\EndIf
\State \textbf{Output:} Accept an offer from the offer book or do nothing.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Buyer Seller's (BS) Decision to Act and Offer and/or Buy Assets}
\begin{algorithmic}[1]
    \State \textbf{Input:} Offer book $O$
    \State \textbf{Buyer Seller Variables:} \textit{Splints}, \textit{Cash}
    \State \textbf{Seller Agent Variables:} \textit{Splints\_seller}, \textit{Cash\_seller}
    \State \textbf{Parameters:} \textit{BS\_sell\_offer\_probability}, \textit{BS\_offer\_ratio}, $a_{BS,l}$, $a_{BS,h}$, $p_{ref}$, \textit{BS\_trading\_probability}, \textit{BS\_search\_length}, \textit{BS\_purchase\_ratio}

    \State \textbf{Pre-trading Phase (Offering as Seller)}:
    \If{$Random(0, 1) < BS\_sell\_offer\_probability$ \textbf{and} $Splints > 0$} 
        \State $n_i \gets BS\_offer\_ratio \times Splints$
        \State $p_i \gets Uniform(a_{BS,l} \times p_{ref}, a_{BS,h} \times p_{ref})$
        \State Add offer $o_i = (p_i, n_i, BS\_Agent)$ to offer book $O$
    \Else
        \State No action taken during pre-trading phase
    \EndIf
    
    \State \textbf{Trading Phase (Buying as Buyer)}:
    \If{$Random(0, 1) < BS\_trading\_probability$}
        \State Filter offers $O_f$ from offer book $O$ where $p_i < p_{ref}$
        \If{$|O_f| > 0$}
            \State \parbox[t]{\linewidth}{Randomly sample \textit{BS\_search\_length} offers from \\ $O_f$}
            \State \parbox[t]{\linewidth}{Choose the offer with the minimum price $o_{min} = \\ (p_{min}, n_{min}, Seller\_Agent)$}
            
            \State \parbox[t]{\linewidth}{Calculate purchase amount $purchase\_amount \gets \\ BS\_purchase\_ratio \times Cash$}
            
            \If{$purchase\_amount \geq p_{min} \times n_{min}$}
                \State \textbf{Buyer Seller:}
                    \State Update \textit{Splints} to $(Splints + n_{min})$
                    \State Update \textit{Cashs} to $(Cash - (p_{min} \times n_{min}))$
                
                \State \textbf{Seller Agent:}
                    \State \parbox[t]{\linewidth}{Update \textit{Splints\_seller} to $(Splints\_seller - \\ n_{min})$}
                    \State \parbox[t]{\linewidth}{Update \textit{Cash\_seller} to $(Cash\_seller + (p_{min} \times \\ n_{min}))$}
                    
                \State Remove $o_{min}$ from $O$
            \Else 
                \State \textbf{Buyer Seller:}
                    \State \parbox[t]{\linewidth}{Update \textit{Splints} to $(Splints + \\ purchase\_amount / p_{min})$}
                    \State Update \textit{Cash} to $(Cash - purchase\_amount)$
                
                \State \textbf{Seller Agent:}
                    \State \parbox[t]{\linewidth}{Update \textit{Splints\_seller} to $(Splints\_seller - \\ (purchase\_amount / p_{min}))$}
                    \State \parbox[t]{\linewidth}{Update \textit{Cash\_seller} to $(Cash\_seller + \\ purchase\_amount)$}
                
                \State \parbox[t]{\linewidth}{Update $n_{min}$ to $(n_{min} - (purchase\_amount \\ / p_{min}))$}
            \EndIf
        \Else
            \State No suitable offers found for purchase
        \EndIf
    \Else
        \State No action taken during trading window
    \EndIf
    
\State \textbf{Output:} Enter an offer in the offer book, accept an offer from the offer book, or do nothing.
\end{algorithmic}
\end{algorithm}

